AnonTokens: tracing re-identification attacks through decoy records

Privacy is of the utmost concern when it comes to releasing data to third parties. Data owners rely on anonymization approaches to safeguard the released datasets against re-identification attacks. However, even with strict anonymization in place, re-identification attacks are still a possibility and in many cases a reality. Prior art has focused on providing better anonymization algorithms with minimal loss of information and how to prevent data disclosure attacks. Our approach tries to tackle the issue of tracing re-identification attacks based on the concept of honeytokens, decoy or "bait" records with the goal to lure malicious users. While the concept of honeytokens has been widely used in the security domain, this is the first approach to apply the concept on the data privacy domain. Records with high re-identification risk, called AnonTokens, are inserted into anonymized datasets. This work demonstrates the feasibility, detectability and usability of AnonTokens and provides promising results for data owners who want to apply our approach to real use cases. We evaluated our concept with real large-scale population datasets. The results show that the introduction of decoy tokens is feasible without significant impact on the released dataset.

==> methodology.tex <==
\section{Methodology}

Comprehensive Hospital Abstract Reporting System (CHARS) dataset - CHARS Public Use File, 2014 

re-identification procedure described here: http://dataprivacylab.org/projects/wa/1089-1.pdf

----

UCI adult dataset

\subsection{Feasibility}

\subsection{Realism}

\subsection{Detectability}





==> monitoring.tex <==
\section{Monitoring re-identification attacks}
\label{sec:monitoring}

One challenging question is how to monitor for re-identification attacks. An obvious answer would be to
monitor the press or conferences for material that refers to this kind of attacks, such as the events published
in \cite{Ochoa01reidentificationof,governordeid,netflixreid}.

A source that can be monitored are paste sites, such as Pastebin, Pastie and Slexy.
Examples of datasets scared in such web-sites are trivial to find through popular web search engines.
Authorities and data owner are actively searching for this type of disclosure in order to remove unauthorized data releases.
Few examples that were valid at the moment of writing are:
\begin{itemize}
  \item \url{https://pastebin.com/GV8NazkT}
  \item \url{https://pastebin.com/FfXVWEZy}.
\end{itemize}

Tools like Dump Monitor\footnote{Available at \url{https://github.com/jordan-wright/dumpmon}} or Pastemon\footnote{Available at \url{https://github.com/xme/pastemon}}
can be easily extended and used for searching records of the published anonymised dataset.

Furthermore, there might be the case that the attacker performs lookups on social media platforms to validate the alleged identity of individuals.
Alas, social media and professional web-sites, such as Facebook and LinkedIn, do not currently provide public APIs to spawn alerts when a user profile is found through search APIs.

